Newton-type Methods for Minimax Optimization

Differential games, in particular two-player sequential zero-sum games (a.k.a. minimax optimization), have been an important modeling tool in applied science and received renewed interest in machine learning due to many recent applications, such as adversarial training, generative models and reinforcement learning. However, existing theory mostly focuses on convex-concave functions with few exceptions. In this work, we propose two novel Newton-type algorithms for nonconvex-nonconcave minimax optimization. We prove their local convergence at strict local minimax points, which are surrogates of global solutions. We argue that our Newton-type algorithms nicely complement existing ones in that (a) they converge faster to strict local minimax points; (b) they are much more effective when the problem is ill-conditioned; (c) their computational complexity remains similar. We verify the effectiveness of our Newton-type algorithms through experiments on training GANs which are intrinsically nonconvex and ill-conditioned. Our code is available at https://github.com/watml/min-max-2nd-order.

==> sections/1-intro.tex <==
%!TEX root = ../main.tex
\section{Introduction}
\label{sec:intro}


Differential games have always played an important role in applied science, from its early applications in economics \citep{morgenstern1953theory} to the Lagrangian reformulation in optimization theory and algorithms, and to the recent resurgence in machine learning (ML). Two-player sequential games, \aka minimax optimization, have been the key piece in recent models such as generative adversarial networks (GAN) \citep{goodfellow2014generative, arjovsky2017wasserstein},
adversarial training \citep{ganin2016domain, madry2017towards}, reinforcement learning \citep{du2017stochastic, dai2018sbeed}, federated learning \citep{MohriSS19} and algorithmic fairness \citep{song2019learning}. Solution concepts, most notably Nash equilibria \citep{nash1950equilibrium}, have been invented, for which numerous (in particular first-order stochastic) algorithms such as gradient-descent-ascent (GDA) \citep{arrow1958studies}, extra-gradient (EG) \citep{korpelevich1976extragradient, popov1980modification, mertikopoulos2018optimistic, hsieh2019convergence}, mirror-prox \citep{nemirovski2004prox} have been designed. They largely rely on the utility function to be convex-concave, which modern ML applications do not necessarily satisfy. Complexity lower bounds of first-order algorithms have been obtained for special classes of convex-concave functions \citep{zhang2019lower, ouyang2019lower, ibrahim2019lower}.

%and extensions to cover nonconvex-concave functions have recently started to appear \citep{lin2020nearoptimal}.
%
%When the problem is zero-sum and convex-concave, this problem has been well studied since strong duality holds and it becomes a saddle point problem \citep{DemyanovMalozemov72, nemirovsky1983problem}, or more generally, the problem of finding a Nash equilibrium  for $n$-players. There have been many first-order algorithms for it, including .


Motivated by recent applications in ML, we study nonconvex-nonconcave minimax optimization. The nonconvexity brings two immediate difficulties: (\textbf{a}) global solution concepts no longer apply and we are forced to consider their localized versions; (\textbf{b}) the order of which player moves first becomes consequential, due to the lack of strong duality. How to theoretically and algorithmically cope with these new challenges has become a hot research topic, of which we mention the differential Stackelberg equilibrium \citep{fiez2019convergence}, the local minimaximality \citep{jin2019minmax, wang2019solving, zhang2020optimality} and the proximal equilibrium \citep{farnia2020gans}. Many algorithms, old and new, have been thoroughly tested, especially by researchers interested in training GANs. Our main goal in this work is to provide an informative comparison of popular algorithms for solving nonconvex-nonconcave minimax problems, point out their connections to two novel Newton-type algorithms, and offer insights on their respective convergence properties.
%Due to the non-convex formulations of recent applications, there has been significant interest in studying non-convex games. Important concepts arise that generalize a local Nash equilibrium, such as the differential Stackelberg equilibrium \citep{fiez2019convergence}, the local minimax point \citep{jin2019minmax, zhang2020optimality}, the generalized local point \citep{zhang2020optimality} and the proximal equilibrium \citep{farnia2020gans}. Such new definitions describe local optimality in the non-convex settings that may arise in real applications \citep[e.g.][]{fiez2019convergence, wang2019solving, farnia2020gans}, and impose new challenges for devising algorithms to converge to these solution concepts.
%since directly applying algorithms in convex games may not work for non-convex games.

% As observed in \cite{zhang2020optimality}, there exist a game and a local minimax where no one-time-scale algorithms would converge to such a point.\todoy{What is a game? What is ``a local minimax''?} By modifying gradient algorithms to two-time-scale, EG/OGD could converge to such local minimax points, but continuous approximation would fail.\todoy{What is two-time-scale? What is EG/OGD?}

In some sense, algorithms aiming to solve nonconvex-nonconcave minimax problems are based on a classic idea that goes back to (at least) Uzawa \cite{arrow1958studies}: iteratively we fix the player that moves first (\aka leader) and call some algorithm \Fa to find a solution for the other player (\aka follower), and then we fix the follower and call some algorithm \La to update the leader's solution. 
%Recent works \citep[\egg][]{fiez2019convergence,jin2019minmax} have proposed relaxation that are more realistic in our nonconvex setting, and 
Many existing algorithms can be treated as an \emph{inexact} implementation of Uzawa's approach, where \Fa need not find an optimal follower solution (\ie best response), particularly so for our nonconvex setting \citep[\egg][]{fiez2019convergence,jin2019minmax}.  The key is to allow \Fa to \emph{adapt quickly} to the update in \La, and some (non-exhaustive) possibilities include:
\begin{itemize}[leftmargin = *, topsep=0pt, itemsep=0pt]
\item Use a larger step size for \Fa and a smaller step size for \La, known as two-time-scale \citep{Borkar08, heusel2017gans,jin2019minmax}; 
\item Perform $k$ steps of \Fa after every step of \La, known (in the GAN literature) as unrolling \citep{metz2016unrolled};
\item Use a faster algorithm (\egg Newton) for \Fa and a slower algorithm (\egg gradient) for \La.
\end{itemize}
Surprisingly, the last scheme above has not been thoroughly studied for nonconvex-nonconcave minimax problems, especially for the new solution concepts such as differential Stackelberg equilibrium \citep{fiez2019convergence} and local minimaximality \citep{jin2019minmax}. In \S\ref{sec:gdn} we fill this gap and propose a novel algorithm, GDN, where \La and \Fa perform gradient and Newton update, respectively. GDN is (locally) as good as unrolling gradient updates even infinitely many times (essentially reducing to Uzawa's original \emph{exact} approach), and recent algorithms such as total gradient descent ascent (TGDA) \citep{fiez2019convergence} and follow-the-ridge (FR) \citep{wang2019solving} can be derived as first-order approximations of GDN and are ``transpose'' of each other, although the three algorithms share the same complexity and all rely on second-order information. We prove the local linear convergence of GDN to (strict) local minimax solutions \citep{fiez2019convergence,jin2019minmax} and demonstrate that for ill-conditioned follower problem, GDN converges much faster%
%than existing alternatives
, much like how Newton's algorithm evades ill-conditioning in conventional minimization problems.

%In this paper we study second-order algorithms for the local convergence near a \emph{strict local minimax} point ({\slmm}), which is also a differential Stackelberg equilibrium \citep{danskin2012theory, basar1999dynamic,fiez2019convergence}. The difficulty is a fast mechanism that changes the follower \emph{quickly} so as to adapt the change of the leader. More specifically, we want to approximately find the best response given the leader's strategy.
% \be\label{eq:best_response}
% \yv' \in \argmax_\yv f(\xv, \yv).
% \en
%In general, such global maximum is hard to find for non-convex (non-concave) problems and we often resort to local maximum as a surrogate. To approximate the best response function, for first-order methods, we can take the step size for the follower to be large and the step size for the leader to be small \citep{jin2019minmax, zhang2020optimality, fiez2019convergence}, or take multiple steps for the follower and one step for the leader \citep{metz2016unrolled}. These first-order methods introduce new hyperparameters that are hard to tune, and convergence rates of first-order methods might be very slow (if they ever converge), as we will see in \Cref{thm:2ts-gda} and in experiments. 

% \begin{table}[t]
%  \centering
% \caption{GD/GA: gradient descent/ascent; SN: Newton update wrt function $f$; EN: Newton update wrt the envelope function $\of_\e$. TGD: total gradient descent. See also \Cref{sec:ingredient} for these acronyms.}% ``2nd order info'' means that the algorithm requires second-order information.}
% \label{tab:algs}
%   \begin{tabular}{llll}
%     \toprule
%     Algorithm  & \texttt{leader} & \texttt{follower} & Comment \\
%     \midrule 
%     2TS-GDA($\a_\La$, $\a_\Fa$) \citep{Borkar08, heusel2017gans,jin2019minmax} & ${\rm GD}(\xv, \a_\La)$ & ${\rm GA}(\yv, \a_\Fa)$ & GDA: $\a_\La = \a_\Fa$ \\
%     UGDA($\a$, $k$) \citep[\egg][]{metz2016unrolled} & ${\rm GD}(\xv, \a)$ & ${\rm GA}(\yv, \a)^k$ & repeating for $k$ times in GA \\
%     TGDA($\a_\La$, $\a_\Fa$) \citep{fiez2019convergence} & ${\rm TGD}(\xv, \a_\La)$ & ${\rm GA}(\yv, \a_\Fa)$ & 2nd order info; linear rate\\
%     FR($\a_\La$, $\a_\Fa$) \citep{wang2019solving} & ${\rm GD}(\xv, \a_\La)$ & ${\rm FR}(\xv, \a_\Fa)$ & 2nd order info; linear rate\\
%     \bf{GDN}($\a_\La$) & ${\rm GD}(\xv, \a_\La)$ & ${\rm SN}(\yv)$ & 2nd order info; linear rate\\
%     \bf{CN} & ${\rm EN}(\xv)$ & ${\rm SN}(\yv)$ & 2nd order info; superlinear rate \\
%     \bottomrule
%   \end{tabular}
%  \vspace{-.7em}
% \end{table}



%Methods that use second-order information have been proposed to accelerate and stabilize the convergence, such as total gradient descent ascent (TGDA) \citep{fiez2019convergence} and follow-the-ridge (FR) \citep{wang2019solving} that use the inverse of Hessian. They can achieve linear convergence near a {\slmm}. However, these methods do not address the ill-conditioning of (the Hessian of) the follower. As we will see in \Cref{sec:second}, when the follower is ill-conditioned, they converge very slowly. In nonlinear optimization, it is well-known that Newton's methods can solve the \emph{ill-conditioning} problem, as they are affine equivariant
%, i.e., $g\circ A = A\circ g$, where $g$ is the Newton's update function and $A$ is an affine transformation 
%\citep[e.g.][]{boyd2004convex}. With this insight, we propose a Newton-type method, which we call \emph{GD-Newton} (GDN), that can avoid the potential ill-conditioning of the follower, and is guaranteed to have faster or equal local linear convergence than TGDA and FR under the same step size choice. There are also methods that do not involve the Hessian inverse including consensus optimization (CO) \citep{mescheder2017numerics}, LOLA \citep{foerster2018learning} and SGA \citep{balduzzi2018mechanics}, but they may not even converge to local minimax points.

Methods such as TGDA, FR and GDN, are still first-order algorithms due to the (slower) gradient update, even though they all use second-order information. These algorithms achieve (local) linear convergence and suffer from the ill-conditioning of the leader problem (and possibly the follower problem too). Fortunately, in \S\ref{sec:second} we show that the Hessian for the leader is also well-defined and we propose a complete Newton (CN) algorithm that performs Newton updates for both the leader and follower. CN enjoys \emph{super-linear} local convergence and evades the ill-conditioning of both leader and follower problems.
%, only linear convergence can be guaranteed as for gradient methods, since these methods essentially use a hybrid of the gradient and the second-order information, which is mainly for acceleration and stability. 
%
%Based on the Hessian information of the leader near a {\slmm}, we provide a much faster Newton's method, called \emph{Complete Newton} (CN), that has \emph{super-linear} local convergence and solves the ill-conditioning of the leader as well. 
To the best of our knowledge, this is the first \emph{genuine} second-order algorithm for nonconvex-nonconcave minimax optimization that (locally) converges super-linearly to (strict) local minimax solutions.
Rather surprisingly, we show that CN, being a second-order algorithm, can be implemented in the same complexity as the first-order alternatives such as TGDA, FR, and GDN.
In \S\ref{sec:exp} we verify our theoretical results and the pros and cons of the proposed Newton-type algorithms by conducting experiments on training GANs. 
%Compared to other algorithms such as TGDA and FR that use second-order information, they have the same computational complexity but much faster convergence rate. These experiments show the potential usage of Newton's methods in minimax optimization.   
We do not include other first-order algorithms such as CO \citep{mescheder2017numerics}, LOLA \citep{foerster2018learning} and SGA \citep{balduzzi2018mechanics} in our study since they may not converge to local minimax solutions. 

\vspace{-.3em}
\paragraph{Contributions}
We summarize the algorithms we study in \Cref{tab:algs}. Near a (strict) local minimax solution, the  convergence rates can be symbolically summarized as follows (larger indicates faster):
\be
\mbox{\bf{CN}} \gg \mbox{\bf{GDN}} = \infty\mbox{-UGDA} \geq \mbox{FR} = \mbox{TGDA} \geq \mbox{2TS-GDA}. 
\en
%In the following subsections we will explore these approximations of best response.
%We list our main contributions:
\begin{itemize}[leftmargin=*, topsep=0pt, itemsep = 0pt]
\item We systematically compare existing algorithms for solving nonconvex-nonconcave minimax problems and provide some revealing connections; 
\item We propose two Newton-type algorithms (GDN and CN) that share the same complexity as existing alternatives but locally converge (much) faster, especially for ill-conditioned problems;
\item We perform experiments on training GANs to complement our theoretical results and to offer some empirical insights on the pros and cons of the aforementioned algorithms.
\end{itemize}

%There are also methods that do not involve the Hessian inverse including 

% We point out that we do not include other first-order algorithms such as consensus optimization (CO) \citep{mescheder2017numerics}, LOLA \citep{foerster2018learning} and SGA \citep{balduzzi2018mechanics} in our study since they may not converge to local minimax solutions. 
% We note that the recent \href{https://github.com/pytorch/pytorch/releases}{release} of PyTorch on new second-order autograd API may greatly simplify the implementation of second-order algorithms and testifies to their potential practical relevance.

